CORE-BEHRT: A Carefully Optimized and Rigorously Evaluated BEHRT

The widespread adoption of Electronic Health Records (EHR) has significantly increased the amount of available healthcare data. This has allowed models inspired by Natural Language Processing (NLP) and Computer Vision, which scale exceptionally well, to be used in EHR research. Particularly, BERT-based models have surged in popularity following the release of BEHRT and Med-BERT. Subsequent models have largely built on these foundations despite the fundamental design choices of these pioneering models remaining underexplored. Through incremental optimization, we study BERT-based EHR modeling and isolate the sources of improvement for key design choices, giving us insights into the effect of data representation, individual technical components, and training procedure. Evaluating this across a set of generic tasks (death, pain treatment, and general infection), we showed that improving data representation can increase the average downstream performance from 0.785 to 0.797 AUROC ($p<10^{-7}$), primarily when including medication and timestamps. Improving the architecture and training protocol on top of this increased average downstream performance to 0.801 AUROC ($p<10^{-7}$). We then demonstrated the consistency of our optimization through a rigorous evaluation across 25 diverse clinical prediction tasks. We observed significant performance increases in 17 out of 25 tasks and improvements in 24 tasks, highlighting the generalizability of our results. Our findings provide a strong foundation for future work and aim to increase the trustworthiness of BERT-based EHR models.

==> figures/data_flowchart.tex <==
\tikzstyle{node} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=orange!30, font=\small]
\tikzstyle{arrow} = [thick,->,>=stealth, font=\small]


\begin{tikzpicture}[node distance=2cm]
\node (start) [node, align=center] {Capital Region of \\ Denmark cohort  \\{} [$1\,825\,101$]};
\node (node1) [node, align=center, right of=start, xshift=3cm] {Patients with \\ diag/med codes \\{} [$1\,805\,176$]};
\node (node2) [node, align=center, right of=node1, xshift=4cm] {Final \\ cohort \\{} [$1\,805\,176$]};

\draw [arrow] (start) -- 
%node[anchor=south, align=center] {Exclude \\ 200000} 
(node1);
\draw [arrow] (node1) -- 
node[anchor=south, align=center]  {Impute \\ missing values} 
node[anchor=north, align=center]  {Exclude \\ incorrect events}
(node2);

\end{tikzpicture}

==> full-paper-template <==
\begin{thebibliography}{53}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[AlSaad et~al.(2022)AlSaad, Malluhi, and Boughorbel]{alsaad2022predict_preterm_birth}
Rawan AlSaad, Qutaibah Malluhi, and Sabri Boughorbel.
\newblock Predictptb: an interpretable preterm birth prediction model using attention-based recurrent neural networks.
\newblock \emph{BioData Mining}, 15\penalty0 (1):\penalty0 6, 2022.

\bibitem[Arboix(2015)]{arboix2015cardiovascular}
Adri{\`a} Arboix.
\newblock Cardiovascular risk factors for acute stroke: Risk profiles in the different subtypes of ischemic stroke.
\newblock \emph{World Journal of Clinical Cases: WJCC}, 3\penalty0 (5):\penalty0 418, 2015.

\bibitem[Asan et~al.(2020)Asan, Bayrak, and Choudhury]{asan2020trust}
Onur Asan, Alparslan~Emrah Bayrak, and Avishek Choudhury.
\newblock Artificial intelligence and human trust in healthcare: Focus on clinicians.
\newblock \emph{J Med Internet Res.}, 2020.

\bibitem[Baevski et~al.(2020)Baevski, Zhou, Mohamed, and Auli]{baevski2020wav2vec2.0}
Alexei Baevski, Henry Zhou, Abdelrahman Mohamed, and Michael Auli.
\newblock wav2vec 2.0: A framework for self-supervised learning of speech representations, 2020.

\bibitem[Booth(1994)]{booth1994read}
Nick Booth.
\newblock What are the read codes?
\newblock \emph{Health libraries review}, 11\penalty0 (3):\penalty0 177--182, 1994.

\bibitem[Chen and Guestrin(2016)]{chen2016xgboost}
Tianqi Chen and Carlos Guestrin.
\newblock Xgboost: A scalable tree boosting system.
\newblock In \emph{Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining}, KDD ’16. ACM, August 2016.
\newblock \doi{10.1145/2939672.2939785}.
\newblock URL \url{http://dx.doi.org/10.1145/2939672.2939785}.

\bibitem[Choi et~al.(2016{\natexlab{a}})Choi, Schuetz, Stewart, and Sun]{choi2016usingrn}
E.~Choi, Andy Schuetz, Walter~F. Stewart, and Jimeng Sun.
\newblock Using recurrent neural network models for early detection of heart failure onset.
\newblock \emph{Journal of the American Medical Informatics Association : JAMIA}, 24:\penalty0 361 -- 370, 2016{\natexlab{a}}.
\newblock URL \url{https://api.semanticscholar.org/CorpusID:3763233}.

\bibitem[Choi et~al.(2015)Choi, Bahadori, and Sun]{choi2015doctorai}
Edward Choi, Mohammad~Taha Bahadori, and Jimeng Sun.
\newblock Doctor {AI:} predicting clinical events via recurrent neural networks.
\newblock \emph{CoRR}, abs/1511.05942, 2015.

\bibitem[Choi et~al.(2016{\natexlab{b}})Choi, Bahadori, Schuetz, Stewart, and Sun]{choi2016retain}
Edward Choi, Mohammad~Taha Bahadori, Andy Schuetz, Walter~F. Stewart, and Jimeng Sun.
\newblock {RETAIN:} interpretable predictive model in healthcare using reverse time attention mechanism.
\newblock \emph{CoRR}, abs/1608.05745, 2016{\natexlab{b}}.

\bibitem[Chowdhery et~al.(2022)Chowdhery, Narang, Devlin, Bosma, Mishra, Roberts, Barham, Chung, Sutton, Gehrmann, Schuh, Shi, Tsvyashchenko, Maynez, Rao, Barnes, Tay, Shazeer, Prabhakaran, Reif, Du, Hutchinson, Pope, Bradbury, Austin, Isard, Gur-Ari, Yin, Duke, Levskaya, Ghemawat, Dev, Michalewski, Garcia, Misra, Robinson, Fedus, Zhou, Ippolito, Luan, Lim, Zoph, Spiridonov, Sepassi, Dohan, Agrawal, Omernick, Dai, Pillai, Pellat, Lewkowycz, Moreira, Child, Polozov, Lee, Zhou, Wang, Saeta, Diaz, Firat, Catasta, Wei, Meier-Hellstern, Eck, Dean, Petrov, and Fiedel]{chowdhery2022palm}
Aakanksha Chowdhery, Sharan Narang, Jacob Devlin, Maarten Bosma, Gaurav Mishra, Adam Roberts, Paul Barham, Hyung~Won Chung, Charles Sutton, Sebastian Gehrmann, Parker Schuh, Kensen Shi, Sasha Tsvyashchenko, Joshua Maynez, Abhishek Rao, Parker Barnes, Yi~Tay, Noam Shazeer, Vinodkumar Prabhakaran, Emily Reif, Nan Du, Ben Hutchinson, Reiner Pope, James Bradbury, Jacob Austin, Michael Isard, Guy Gur-Ari, Pengcheng Yin, Toju Duke, Anselm Levskaya, Sanjay Ghemawat, Sunipa Dev, Henryk Michalewski, Xavier Garcia, Vedant Misra, Kevin Robinson, Liam Fedus, Denny Zhou, Daphne Ippolito, David Luan, Hyeontaek Lim, Barret Zoph, Alexander Spiridonov, Ryan Sepassi, David Dohan, Shivani Agrawal, Mark Omernick, Andrew~M. Dai, Thanumalayan~Sankaranarayana Pillai, Marie Pellat, Aitor Lewkowycz, Erica Moreira, Rewon Child, Oleksandr Polozov, Katherine Lee, Zongwei Zhou, Xuezhi Wang, Brennan Saeta, Mark Diaz, Orhan Firat, Michele Catasta, Jason Wei, Kathy Meier-Hellstern, Douglas Eck, Jeff Dean, Slav Petrov, and Noah Fiedel.
\newblock Palm: Scaling language modeling with pathways, 2022.

\bibitem[Dauphin et~al.(2017)Dauphin, Fan, Auli, and Grangier]{dauphin2017glu}
Yann~N. Dauphin, Angela Fan, Michael Auli, and David Grangier.
\newblock Language modeling with gated convolutional networks, 2017.

\bibitem[Dettmers et~al.(2023)Dettmers, Pagnoni, Holtzman, and Zettlemoyer]{dettmers2023qlora}
Tim Dettmers, Artidoro Pagnoni, Ari Holtzman, and Luke Zettlemoyer.
\newblock Qlora: Efficient finetuning of quantized llms, 2023.

\bibitem[Devlin et~al.(2018)Devlin, Chang, Lee, and Toutanova]{devlin2018bert}
Jacob Devlin, Ming-Wei Chang, Kenton Lee, and Kristina Toutanova.
\newblock Bert: Pre-training of deep bidirectional transformers for language understanding.
\newblock \emph{arXiv preprint arXiv:1810.04805}, 2018.

\bibitem[Dosovitskiy et~al.(2021)Dosovitskiy, Beyer, Kolesnikov, Weissenborn, Zhai, Unterthiner, Dehghani, Minderer, Heigold, Gelly, Uszkoreit, and Houlsby]{dosovitskiy2021vit}
Alexey Dosovitskiy, Lucas Beyer, Alexander Kolesnikov, Dirk Weissenborn, Xiaohua Zhai, Thomas Unterthiner, Mostafa Dehghani, Matthias Minderer, Georg Heigold, Sylvain Gelly, Jakob Uszkoreit, and Neil Houlsby.
\newblock An image is worth 16x16 words: Transformers for image recognition at scale, 2021.

\bibitem[He et~al.(2021)He, Chen, Xie, Li, Dollár, and Girshick]{he2021mae}
Kaiming He, Xinlei Chen, Saining Xie, Yanghao Li, Piotr Dollár, and Ross Girshick.
\newblock Masked autoencoders are scalable vision learners, 2021.

\bibitem[Henriksen et~al.(2017)Henriksen, Nordgaard, and Jansson]{henriksen2017genetics_schizophrenia}
Mads~G Henriksen, Julie Nordgaard, and Lennart~B Jansson.
\newblock Genetics of schizophrenia: overview of methods, findings and limitations.
\newblock \emph{Frontiers in human neuroscience}, 11:\penalty0 322, 2017.

\bibitem[Horsky et~al.(2017)Horsky, Drucker, and Ramelson]{horsky2017accuracy_icd10}
Jan Horsky, Elizabeth~A Drucker, and Harley~Z Ramelson.
\newblock Accuracy and completeness of clinical coding using icd-10 for ambulatory visits.
\newblock In \emph{AMIA annual symposium proceedings}, volume 2017, page 912. American Medical Informatics Association, 2017.

\bibitem[Johnson et~al.(2016)Johnson, A., Pollard, T., Shen, and et~al.]{johnson2016mimic3}
Johnson, A., Pollard, T., Shen, and L.~et~al.
\newblock Mimic-iii, a freely accessible critical care database.
\newblock \emph{Scientific Data}, 2016.

\bibitem[Kazemi et~al.(2019)Kazemi, Goel, Eghbali, Ramanan, Sahota, Thakur, Wu, Smyth, Poupart, and Brubaker]{kazemi2019time2vec}
Seyed~Mehran Kazemi, Rishab Goel, Sepehr Eghbali, Janahan Ramanan, Jaspreet Sahota, Sanjay Thakur, Stella Wu, Cathal Smyth, Pascal Poupart, and Marcus Brubaker.
\newblock Time2vec: Learning a vector representation of time, 2019.

\bibitem[Khalilia et~al.(2011)Khalilia, Chakraborty, and Popescu]{khalilia2011predicting_rf}
Mohammed Khalilia, Sounak Chakraborty, and Mihail Popescu.
\newblock Predicting disease risks from highly imbalanced data using random forest.
\newblock \emph{BMC medical informatics and decision making}, 11:\penalty0 1--13, 2011.

\bibitem[Lauritzen et~al.(2023)Lauritzen, von Euler-Chelpin, Lynge, Vejborg, Nielsen, Karssemeijer, and Lillholm]{lauritzen2023assessing}
Andreas~D Lauritzen, My~C von Euler-Chelpin, Elsebeth Lynge, Ilse Vejborg, Mads Nielsen, Nico Karssemeijer, and Martin Lillholm.
\newblock Assessing breast cancer risk by combining ai for lesion detection and mammographic texture.
\newblock \emph{Radiology}, 308\penalty0 (2):\penalty0 e230227, 2023.

\bibitem[Li et~al.(2020)Li, Rao, Solares, Hassaine, Ramakrishnan, Canoy, Zhu, Rahimi, and Salimi-Khorshidi]{li2020behrt}
Yikuan Li, Shishir Rao, Jos{\'e} Roberto~Ayala Solares, Abdelaali Hassaine, Rema Ramakrishnan, Dexter Canoy, Yajie Zhu, Kazem Rahimi, and Gholamreza Salimi-Khorshidi.
\newblock Behrt: transformer for electronic health records.
\newblock \emph{Scientific reports}, 10\penalty0 (1):\penalty0 1--12, 2020.

\bibitem[Li et~al.(2022)Li, Mamouei, Salimi-Khorshidi, Rao, Hassaine, Canoy, Lukasiewicz, and Rahimi]{li2022hibehrt}
Yikuan Li, Mohammad Mamouei, Gholamreza Salimi-Khorshidi, Shishir Rao, Abdelaali Hassaine, Dexter Canoy, Thomas Lukasiewicz, and Kazem Rahimi.
\newblock Hi-behrt: Hierarchical transformer-based model for accurate prediction of clinical events using multimodal longitudinal electronic health records.
\newblock \emph{IEEE Journal of Biomedical and Health Informatics}, 2022.

\bibitem[Liu et~al.(2019)Liu, Ott, Goyal, Du, Joshi, Chen, Levy, Lewis, Zettlemoyer, and Stoyanov]{liu2019roberta}
Yinhan Liu, Myle Ott, Naman Goyal, Jingfei Du, Mandar Joshi, Danqi Chen, Omer Levy, Mike Lewis, Luke Zettlemoyer, and Veselin Stoyanov.
\newblock Roberta: A robustly optimized bert pretraining approach, 2019.

\bibitem[Mahajan et~al.(2018)Mahajan, Girshick, Ramanathan, He, Paluri, Li, Bharambe, and van~der Maaten]{mahajan2018sqrt}
Dhruv Mahajan, Ross~B. Girshick, Vignesh Ramanathan, Kaiming He, Manohar Paluri, Yixuan Li, Ashwin Bharambe, and Laurens van~der Maaten.
\newblock Exploring the limits of weakly supervised pretraining.
\newblock \emph{CoRR}, abs/1805.00932, 2018.
\newblock URL \url{http://arxiv.org/abs/1805.00932}.

\bibitem[Mikolov et~al.(2013)Mikolov, Sutskever, Chen, Corrado, and Dean]{mikolov2013nlpsqrt}
Tom{\'{a}}s Mikolov, Ilya Sutskever, Kai Chen, Greg Corrado, and Jeffrey Dean.
\newblock Distributed representations of words and phrases and their compositionality.
\newblock \emph{CoRR}, abs/1310.4546, 2013.
\newblock URL \url{http://arxiv.org/abs/1310.4546}.

\bibitem[MJ et~al.(1997)MJ, TE, DM, BH, LA, DE, CM, TJ, and WN]{fine1997logisticregression}
Fine MJ, Auble TE, Yealy DM, Hanusa BH, Weissfeld LA, Singer DE, Coley CM, Marrie TJ, and Kapoor WN.
\newblock A prediction rule to identify low-risk patients with community-acquired pneumonia.
\newblock \emph{N Engl J Med.}, 1997.

\bibitem[Montagnon et~al.(2020)Montagnon, Cerny, Cadrin-Ch{\^e}nevert, Hamilton, Derennes, Ilinca, Vandenbroucke-Menu, Turcotte, Kadoury, and Tang]{montagnon2020deep_radiology}
Emmanuel Montagnon, Milena Cerny, Alexandre Cadrin-Ch{\^e}nevert, Vincent Hamilton, Thomas Derennes, Andr{\'e} Ilinca, Franck Vandenbroucke-Menu, Simon Turcotte, Samuel Kadoury, and An~Tang.
\newblock Deep learning workflow in radiology: a primer.
\newblock \emph{Insights into imaging}, 11:\penalty0 1--15, 2020.

\bibitem[Nguyen et~al.(2016)Nguyen, Tran, Wickramasinghe, and Venkatesh]{nguyen2016deepr}
Phuoc Nguyen, Truyen Tran, Nilmini Wickramasinghe, and Svetha Venkatesh.
\newblock $\backslash$ mathtt $\{$Deepr$\}$ : a convolutional net for medical records.
\newblock \emph{IEEE journal of biomedical and health informatics}, 21\penalty0 (1):\penalty0 22--30, 2016.

\bibitem[Nourazari et~al.(2021)Nourazari, Davis, Granovsky, Austin, Straff, Joseph, and Sanchez]{nourazari2021decreased}
Sara Nourazari, Samuel~R Davis, Rachel Granovsky, Randolph Austin, Dean~J Straff, Joshua~W Joseph, and Leon~D Sanchez.
\newblock Decreased hospital admissions through emergency departments during the covid-19 pandemic.
\newblock \emph{The American journal of emergency medicine}, 42:\penalty0 203--210, 2021.

\bibitem[Pang et~al.(2021)Pang, Jiang, Kalluri, Spotnitz, Chen, Perotte, and Natarajan]{pang2021cehr}
Chao Pang, Xinzhuo Jiang, Krishna~S Kalluri, Matthew Spotnitz, RuiJun Chen, Adler Perotte, and Karthik Natarajan.
\newblock Cehr-bert: Incorporating temporal information from structured ehr data to improve prediction tasks.
\newblock In \emph{Machine Learning for Health}, pages 239--260. PMLR, 2021.

\bibitem[Prakash et~al.(2021)Prakash, Chilukuri, Ranade, and Viswanathan]{prakash2021rarebert}
P.~Prakash, S.~Chilukuri, N.~Ranade, and S.~Viswanathan.
\newblock Rarebert: Transformer architecture for rare disease patient identification using administrative claims.
\newblock \emph{Proceedings of the AAAI Conference on Artificial Intelligence}, 2021.

\bibitem[Ramachandran et~al.(2017)Ramachandran, Zoph, and Le]{ramachandran2017swish}
Prajit Ramachandran, Barret Zoph, and Quoc~V. Le.
\newblock Searching for activation functions, 2017.

\bibitem[Rao et~al.(2022)Rao, Mamouei, Salimi-Khorshidi, Li, Ramakrishnan, Hassaine, Canoy, and Rahimi]{rao2022targetedbehrt}
Shishir Rao, Mohammad Mamouei, Gholamreza Salimi-Khorshidi, Yikuan Li, Rema Ramakrishnan, Abdelaali Hassaine, Dexter Canoy, and Kazem Rahimi.
\newblock Targeted-behrt: Deep learning for observational causal inference on longitudinal electronic health records.
\newblock \emph{IEEE Transactions on Neural Networks and Learning Systems}, 2022.

\bibitem[Rasmy et~al.(2021)Rasmy, Xiang, Xie, Tao, and Zhi]{rasmy2021medbert}
Laila Rasmy, Yang Xiang, Ziqian Xie, Cui Tao, and Degui Zhi.
\newblock Med-bert: pretrained contextualized embeddings on large-scale structured electronic health records for disease prediction.
\newblock \emph{NPJ digital medicine}, 4\penalty0 (1):\penalty0 86, 2021.

\bibitem[Schuster and Paliwal(1997)]{schuster1997bidirectional}
Mike Schuster and Kuldip~K Paliwal.
\newblock Bidirectional recurrent neural networks.
\newblock \emph{IEEE transactions on Signal Processing}, 45\penalty0 (11):\penalty0 2673--2681, 1997.

\bibitem[Shang et~al.(2019)Shang, Ma, Xiao, and Sun]{shang2019gbert}
Junyuan Shang, Tengfei Ma, Cao Xiao, and Jimeng Sun.
\newblock Pre-training of graph augmented transformers for medication recommendation.
\newblock \emph{arXiv preprint arXiv:1906.00346}, 2019.

\bibitem[Shazeer(2020)]{shazeer2020glu}
Noam Shazeer.
\newblock Glu variants improve transformer, 2020.

\bibitem[Slawomirski et~al.(2023)Slawomirski, Lindner, de~Bienassis, Haywood, Hashiguchi, Steentjes, and Oderkirk]{slawomirski2023progress}
Luke Slawomirski, Luca Lindner, Katherine de~Bienassis, Philip Haywood, Tiago Cravo~Oliveira Hashiguchi, Melanie Steentjes, and Jillian Oderkirk.
\newblock Progress on implementing and using electronic health record systems: Developments in oecd countries as of 2021.
\newblock \emph{OECD Health Working Papers}, 2023.

\bibitem[Stilo and Murray(2019)]{stilo2019non_genetic_schizophrenia}
Simona~A Stilo and Robin~M Murray.
\newblock Non-genetic factors in schizophrenia.
\newblock \emph{Current psychiatry reports}, 21:\penalty0 1--10, 2019.

\bibitem[Su et~al.(2023)Su, Lu, Pan, Murtadha, Wen, and Liu]{su2023roformer}
Jianlin Su, Yu~Lu, Shengfeng Pan, Ahmed Murtadha, Bo~Wen, and Yunfeng Liu.
\newblock Roformer: Enhanced transformer with rotary position embedding, 2023.

\bibitem[Teoh(2018)]{teoh2018towards_stroke_prediction}
Douglas Teoh.
\newblock Towards stroke prediction using electronic health records.
\newblock \emph{BMC medical informatics and decision making}, 18:\penalty0 1--11, 2018.

\bibitem[Tong et~al.(2022)Tong, Song, Wang, and Wang]{tong2022videomae}
Zhan Tong, Yibing Song, Jue Wang, and Limin Wang.
\newblock Videomae: Masked autoencoders are data-efficient learners for self-supervised video pre-training, 2022.

\bibitem[Touvron et~al.(2023)Touvron, Lavril, Izacard, Martinet, Lachaux, Lacroix, Rozière, Goyal, Hambro, Azhar, Rodriguez, Joulin, Grave, and Lample]{touvron2023llama}
Hugo Touvron, Thibaut Lavril, Gautier Izacard, Xavier Martinet, Marie-Anne Lachaux, Timothée Lacroix, Baptiste Rozière, Naman Goyal, Eric Hambro, Faisal Azhar, Aurelien Rodriguez, Armand Joulin, Edouard Grave, and Guillaume Lample.
\newblock Llama: Open and efficient foundation language models, 2023.

\bibitem[V et~al.(2019)V, S, A, K, O, S, S, M, D, CA, RT, R, R, JP, ICK, H, and AD]{kuan2019caliber}
Kuan V, Denaxas S, Gonzalez-Izquierdo A, Direk K, Bhatti O, Husain S, Sutaria S, Hingorani M, Nitsch D, Parisinos CA, Lumbers RT, Mathur R, Sofat R, Casas JP, Wong ICK, Hemingway H, and Hingorani AD.
\newblock A chronological map of 308 physical and mental health conditions from 4 million individuals in the english national health service.
\newblock \emph{Lancet Digit Health}, 2019.

\bibitem[Vaswani et~al.(2017)Vaswani, Shazeer, Parmar, Uszkoreit, Jones, Gomez, Kaiser, and Polosukhin]{vaswani2017attention}
Ashish Vaswani, Noam Shazeer, Niki Parmar, Jakob Uszkoreit, Llion Jones, Aidan~N Gomez, {\L}ukasz Kaiser, and Illia Polosukhin.
\newblock Attention is all you need.
\newblock \emph{Advances in neural information processing systems}, 30, 2017.

\bibitem[Wei et~al.(2016)Wei, Teixeira, Mo, Cronin, Warner, and Denny]{wei2016combining_ehr}
Wei-Qi Wei, Pedro~L Teixeira, Huan Mo, Robert~M Cronin, Jeremy~L Warner, and Joshua~C Denny.
\newblock Combining billing codes, clinical notes, and medications from electronic health records provides superior phenotyping performance.
\newblock \emph{Journal of the American Medical Informatics Association}, 23\penalty0 (e1):\penalty0 e20--e27, 2016.

\bibitem[Wettig et~al.(2023)Wettig, Gao, Zhong, and Chen]{wettig2023mask}
Alexander Wettig, Tianyu Gao, Zexuan Zhong, and Danqi Chen.
\newblock Should you mask 15% in masked language modeling?, 2023.

\bibitem[Wu et~al.(2017)Wu, Burnside, Cox, Fan, Yuan, Yin, Peissig, Cobian, Page, and Craven]{wu2017breast_cancer}
Yirong Wu, Elizabeth~S Burnside, Jennifer Cox, Jun Fan, Ming Yuan, Jie Yin, Peggy Peissig, Alexander Cobian, David Page, and Mark Craven.
\newblock Breast cancer risk prediction using electronic health records.
\newblock In \emph{2017 IEEE International Conference on Healthcare Informatics (ICHI)}, pages 224--228. IEEE, 2017.

\bibitem[Y et~al.(2021)Y, W, MK, and CW.]{meng2021brltm}
Meng Y, Speier W, Ong MK, and Arnold CW.
\newblock Bidirectional representation learning from transformers using multimodal electronic health record data to predict depression.
\newblock \emph{IEEE Journal of Biomedical and Health Informatics}, 2021.

\bibitem[Yang et~al.(2019)Yang, Dai, Yang, Carbonell, Salakhutdinov, and Le]{yang2019xlnet}
Zhilin Yang, Zihang Dai, Yiming Yang, Jaime Carbonell, Russ~R Salakhutdinov, and Quoc~V Le.
\newblock Xlnet: Generalized autoregressive pretraining for language understanding.
\newblock \emph{Advances in neural information processing systems}, 32, 2019.

\bibitem[Yasaka and Abe(2018)]{yasaka2018deep_radiology}
Koichiro Yasaka and Osamu Abe.
\newblock Deep learning and artificial intelligence in radiology: Current applications and future directions.
\newblock \emph{PLoS medicine}, 15\penalty0 (11):\penalty0 e1002707, 2018.

\bibitem[Zhang et~al.(2022)Zhang, Chen, and Bui]{zhang2022adadiag}
Tianran Zhang, Muhao Chen, and Alex~A.T. Bui.
\newblock Adadiag: Adversarial domain adaptation of diagnostic prediction with clinical event sequences,.
\newblock \emph{Journal of Biomedical Informatics}, 2022.

\end{thebibliography}


==> tables/cohort_stats_table.tex <==
\begin{table}[!h]
\caption{Statistics for the CV sets for all 25 downstream tasks for diagnosis+medication data. Trajectory length (first encounter until censoring) is given in days, and the sequence length is defined as the number of events in a patients sequence (after censoring).}
\begin{tabular}{
p{0.22\linewidth}
>{\centering\arraybackslash}p{0.14\linewidth}
p{0.15\linewidth}
p{0.175\linewidth}
>{\centering\arraybackslash}p{0.1\linewidth}
>{\centering\arraybackslash}p{0.09\linewidth}
}
    \toprule
    Condition & Age (mean±std) & Sequence\newline Length\newline Q2(Q1-Q3) & Trajectory Length\newline Q2(Q1-Q3) & \multicolumn{2}{>{\centering\arraybackslash}p{0.09\linewidth}}{Patients\newline [thousands]/\newline Prevalence[\%]} \\
    \midrule
    Alzheimer's\newline Disease & 79.1±7.1 & 27 (3-161) & 917 (471-1437) & \dualcol{46.2}{3.7} \\
    Anaphylaxis & 41.6±24.7 & 4 (1-28) & 813 (381-1281) & \dualcol{338.1}{0.2} \\
    Arrhythmia & 73.6±9.2 & 9 (2-85) & 890 (516-1366) & \dualcol{70.9}{10.7} \\
    Basal Cell\newline Carcinoma & 79.4±7.2 & 22 (3-147) & 1093 (710-1571) & \dualcol{41.2}{4.6} \\
    Breast Cancer & 74.4±9.6 & 11 (2-102) & 852 (443-1395) & \dualcol{27.1}{4.5} \\
    Colon Cancer & 73.7±9.3 & 14 (2-110) & 875 (464-1407) & \dualcol{71.0}{1.3} \\
    Lung Cancer & 73.7±9.2 & 14 (2-110) & 880 (461-1407) & \dualcol{69.9}{2.1} \\
    Pancreatic Cancer & 73.7±9.3 & 15 (3-117) & 903 (486-1403) & \dualcol{75.5}{0.4} \\
    Death & 73.7±9.1 & 11 (2-89) & 1092 (713-1565) & \dualcol{70.1}{22.5} \\
    Depression & 22.5±4.3 & 2 (1-7) & 752 (391-1235) & \dualcol{53.5}{2.7} \\
    Diabetes & 41.9±24.7 & 3 (1-17) & 715 (411-1143) & \dualcol{214.8}{5.0} \\
    Diarrhea & 41.5±24.7 & 4 (1-26) & 676 (315-1137) & \dualcol{316.3}{1.3} \\
    Infection & 41.2±24.7 & 2 (1-7) & 516 (201-995) & \dualcol{281.9}{42.6} \\
    Major Bleeding & 41.7±24.7 & 4 (1-26) & 732 (341-1238) & \dualcol{325.1}{4.7} \\
    Myocardial\newline Infarction & 73.7±9.3 & 16 (3-118) & 845 (420-1366) & \dualcol{80.8}{2.7} \\
    Osteonecrosis & 79.4±7.2 & 32 (4-176) & 1105 (643-1597) & \dualcol{51.4}{0.2} \\
    Pain Treatment & 40.8±24.5 & 2 (1-5) & 497 (212-919) & \dualcol{267.5}{42.0} \\
    Pneumonia & 41.7±24.8 & 4 (1-24) & 655 (302-1190) & \dualcol{293.2}{5.5} \\
    Large Fetus & 30.4±5.1 & 3 (2-7) & 168 (0-778) & \dualcol{22.2}{2.3} \\
    Placental\newline Insufficiency & 30.4±5.0 & 3 (2-7) & 160 (0-778) & \dualcol{22.2}{80.6} \\
    Fetal Growth\newline Disorder & 30.4±5.1 & 3 (2-7) & 162 (0-775) & \dualcol{22.2}{6.6} \\
    Preterm Birth& 30.4±5.0 & 3 (2-7) & 161 (0-782) & \dualcol{22.2}{13.7} \\
    Schizophrenia & 24.7±2.9 & 2 (1-7) & 568 (284-1066) & \dualcol{25.5}{1.2} \\
    Sleep Disorder & 29.3±5.6 & 2 (1-11) & 662 (358-1061) & \dualcol{67.9}{4.3} \\
    Stroke & 73.5±9.1 & 12 (2-102) & 709 (325-1284) & \dualcol{60.4}{1.4} \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/group_definition_table.tex <==
\begin{table}[ht!]\label{tab}
\centering
\caption{Comprehensive table of conditions with specified age group and prediction window. for sleep disorder age dist: \cite{grandner2012age_sleep_disorder} }
\begin{tabular}{p{0.35\linewidth}p{0.25\linewidth}p{0.25\linewidth}}
    \toprule
    Disease & Group & Prediction\newline Window \\
    \midrule
    \textbf{Death} & 60+ y.o.& 1 year \\%x 
    \textbf{Infection} & all & 7 days \\%x
    \textbf{Pain treatment} & all & 30 days \\%x
    \textbf{Cancer}  \\
    \quad Basal cell carcinoma & 70+ y.o. & 1 year \\ %x
    \quad Breast cancer & women 60+ y.o. & 3 months \\%x
    \quad Colon cancer & 60+ y.o. & 3 months \\%x
    \quad Lung cancer & 60+ y.o. & 3 months \\%x
    \quad Pancreatic cancer & 60+ y.o. & 3 months \\%x
    \textbf{Chronic} \\
    \quad Alzheimer's & 70+ y.o. & 3 months \\%x
    \quad Arrhythmia & 60+ y.o. & 6 months \\ %x
    \quad Diabetes & All & 6 months \\ %x
    \quad Osteonecrosis & 70+ y.o. & 6 months \\ %x
    \textbf{Acute and Emergencies} \\
    \quad Anaphylaxis & all & 24 hours \\%x
    \quad Diarrhea & all & 3 days \\ %x
    \quad Major bleeding & all & 24 hours \\ %x
    \quad Myocardial Infarction & 60+ y.o. & 14 days \\ %x
    %\quad Hip Fracture & 70+ y.o. & 6 months \\ % need to create outcome
    \quad Pneumonia & all & 14 days \\ %x
    \quad Stroke & 60+ y.o. & 14 days \\ %x
    \textbf{Psychiatric} \\
    \quad Schizophrenia & 20-30 & 3 months \\
    \quad Depression & 15-30 & 3 months \\ % check age distribution
    \textbf{Pregnancy-Related} \\
    \quad Preterm birth & pregnant & at pregnacny \\ %x
    \quad FGR & pregnant & at pregnacny \\%x 
    \quad Placental ins. & pregnant & at pregnacny \\%x
    \quad Fetal Macrosomia & pregnant & at pregnacny \\%x
    %\quad Hydramnion & pregnant  & at pregnacny \\ % save for later
    %\quad Oligohydramnion & pregnant  & at pregnacny \\ %save for later
    \textbf{Others} \\
    \quad Sleep disorder & 20-40 y.o. & 3 months \\ %x
    %quad Vacc. granuloma & 0-18 y.o. & 3 months \\
    %\quad Steven Johnson synd. & all & 1 month \\
    \bottomrule
\end{tabular}\label{tab:task_info}
\end{table}

==> tables/initial_exp_results.tex <==
\begin{table}[H]
\caption{Performance in initial experiments given as AUROC and AUPRC scores in predicting Pain, Death, and Infection}
\label{tab:model_stats}
\centering
\begin{tabular}{|l|ccc|ccc|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{AUROC (\%)} & \multicolumn{3}{c|}{AUPRC (\%)} \\
\cline{2-7}
& Pain & Death & Infection & Pain & Death & Infection \\
\hline
MedBERT & 76.5$\pm$0.1 & 79.2$\pm$0.1 & 72.7$\pm$0.1 & 79.1$\pm$0.1 & 52.8$\pm$0.2 & 77.9$\pm$0.1 \\
BEHRT & 77.0$\pm$0.1 & 84.5$\pm$0.1 & 73.9$\pm$0.1 & 79.5$\pm$0.2 & 60.3$\pm$0.4 & 78.8$\pm$0.1 \\
+Med & 77.7$\pm$0.1 & 84.6$\pm$0.1 & 74.4$\pm$0.1 & 80.2$\pm$0.1 & 60.9$\pm$0.2 & 79.5$\pm$0.1 \\
+FV+Sex & 77.9$\pm$0.1 & 84.7$\pm$0.2 & 74.3$\pm$0.0 & 80.4$\pm$0.1 & 61.2$\pm$0.4 & 79.4$\pm$0.1 \\
-SEP & 77.8$\pm$0.0 & 84.2$\pm$0.2 & 74.4$\pm$0.1 & 80.3$\pm$0.0 & 61.1$\pm$0.4 & 79.3$\pm$0.1 \\
Simplified Segments & 78.1$\pm$0.0 & 84.6$\pm$0.2 & 74.4$\pm$0.2 & 80.5$\pm$0.0 & 61.1$\pm$0.3 & 79.3$\pm$0.2 \\
+time2vec(abspos) & 78.5$\pm$0.1 & 85.6$\pm$0.1 & 75.1$\pm$0.1 & 80.9$\pm$0.1 & 63.4$\pm$0.3 & 80.3$\pm$0.1 \\
+time2vec(age) & 78.5$\pm$0.0 & 85.7$\pm$0.1 & 75.2$\pm$0.1 & 80.9$\pm$0.0 & 63.7$\pm$0.3 & 80.3$\pm$0.1 \\
\parbox[t]{5cm}{+RoPE\newline+SwiGLU}& 78.5$\pm$0.1 & 85.6$\pm$0.1 & 75.4$\pm$0.1 & 80.8$\pm$0.1 & 63.6$\pm$0.4 & 80.6$\pm$0.2 \\
Masking Ratio 10\% & 78.4$\pm$0.1 & 85.5$\pm$0.1 & 75.2$\pm$0.1 & 80.8$\pm$0.1 & 63.4$\pm$0.2 & 80.3$\pm$0.2 \\
Masking Ratio 20\% & 78.7$\pm$0.1 & 85.7$\pm$0.1 & 75.5$\pm$0.2 & 81.0$\pm$0.1 & 63.9$\pm$0.2 & 80.6$\pm$0.1 \\
Masking Ratio 25\% & 78.6$\pm$0.1 & 85.9$\pm$0.1 & 75.2$\pm$0.1 & 80.9$\pm$0.1 & 64.2$\pm$0.2 & 80.4$\pm$0.1 \\
Masking Ratio 30\% & 78.6$\pm$0.1 & 85.7$\pm$0.2 & 75.4$\pm$0.1 & 80.9$\pm$0.0 & 63.9$\pm$0.4 & 80.4$\pm$0.1 \\
Masking Ratio 50\% & 78.2$\pm$0.0 & 85.2$\pm$0.2 & 74.7$\pm$0.1 & 80.6$\pm$0.0 & 63.3$\pm$0.3 & 79.8$\pm$0.1 \\
Masking Ratio 20\% \newline + PLOS & 78.6$\pm$0.1 & 85.6$\pm$0.1 & 75.6$\pm$0.1 & 80.9$\pm$0.1 & 63.4$\pm$0.4 & 80.6$\pm$0.1 \\
Max Pooling & 78.7$\pm$0.1 & 85.7$\pm$0.1 & 75.4$\pm$0.1 & 81.1$\pm$0.0 & 64.1$\pm$0.1 & 80.6$\pm$0.1 \\
Mean Pooling & 78.6$\pm$0.1 & 85.9$\pm$0.1 & 75.7$\pm$0.1 & 81.1$\pm$0.0 & 63.9$\pm$0.3 & 80.9$\pm$0.1 \\
Sum Pooling & xx.x$\pm$xx & xx.x$\pm$x.x & xx.x$\pm$x.x & xx.x$\pm$x.x & xx.x$\pm$x.x & xx.x$\pm$x.x \\
Weighted Attention & 78.8$\pm$0.1 & 85.8$\pm$0.1 & 75.7$\pm$0.1 & 81.2$\pm$0.1 & 63.6$\pm$0.1 & 80.8$\pm$0.1 \\
BiLSTM & 78.7$\pm$0.1 & 85.7$\pm$0.1 & 75.5$\pm$0.1 & 81.1$\pm$0.1 & 64.2$\pm$0.2 & 80.6$\pm$0.1 \\
BiGRU & 78.7$\pm$0.1 & 85.9$\pm$0.1 & 75.7$\pm$0.1 & 81.2$\pm$0.1 & 63.9$\pm$0.3 & 80.9$\pm$0.1 \\
\hline
\end{tabular}
\end{table}

==> tables/main_table.tex <==
\begin{table}[ht!]
\centering
 \caption{Model performance for base, base+ and best model for multiple conditions alongside demographics for positive patients in the test set.\newline$^{*/**/***}\,$ Model is significantly better than base model $p<0.05/0.01/0.001$}
\begin{tabular}{p{0.22\linewidth}p{0.13\linewidth}p{0.08\linewidth}p{0.14\linewidth}p{0.14\linewidth}p{0.14\linewidth}}
    \toprule
    Disease & Age & \% Male & AUROC\newline base  &AUROC\newline base+&AUROC \newline best  \\
    \midrule    
    \textbf{Cancer} \\
    \quad Basal cell\newline carcinoma & 80.1±6.6 & 50 & 0.644±0.004 & xx±xx & 0.672±0.009** \\
    \quad Breast cancer & 73.9±8.7 & 0 & 0.570±0.075 & xx±xx & 0.624±0.005 \\
    \quad Colon cancer & 75.1±8.0 & 55 & 0.614±0.007 & xx±xx & 0.628±0.025 \\
    \quad Lung cancer & 73.5±6.8 & 46 & 0.665±0.004 & xx±xx & 0.684±0.003** \\
    \quad Pancreatic cancer & 74.1±7.9 & 53 & 0.529±0.057 & xx±xx & 0.565±0.032 \\
    \textbf{Cardiovascular}\\
    \quad Arrhythmia & 76.1±8.7 & 50 & 0.689±0.002 & xx±xx & 0.716±0.001*** \\
    \quad MI & 74.6±8.7 & 63 & 0.657±0.003 & xx±xx & 0.687±0.003*** \\
    \quad Stroke & 75.4±9.0 & 53 & 0.645±0.011 & xx±xx & 0.702±0.008*** \\
    \textbf{Chronic} \\
    \quad Alzheimer's & 81.6±6.2 & 43 & 0.739±0.004 & xx±xx & 0.770±0.005*** \\
    \quad Diabetes & 65.1±16.4 & 57 & 0.835±0.001 & xx±xx & 0.848±0.002*** \\
    \quad Osteonecrosis & 77.2±5.5 & 36 & 0.825±0.050 & xx±xx & 0.842±0.038 \\
    \textbf{Death} & 80.3±9.7 & 51 & 0.866±0.0003 & xx±xx & 0.877±0.001*** \\
    \textbf{Emergencies} \\
    \quad Anaphylaxis & 32.1±25.5 & 34 & 0.710±0.014 & xx±xx & 0.719±0.009 \\
    \quad Diarrhea & 59.0±23.5 & 46 & 0.856±0.002 & xx±xx & 0.875±0.005** \\
    \quad Major bleeding & 59.3±23.8 & 54 & 0.782±0.001 & xx±xx & 0.797±0.002*** \\
    \textbf{Infectionns}\\
    \quad Infections & 46.8±26.3 & 44 & xx±xx & xx±xx & xx±xx \\
    \quad Pneumonia & 60.9±26.8 & 51 & 0.8228±0.0007 & xx±xx & 0.8323±0.0013 \\
    \textbf{Psychiatric} \\
    \quad Depression & 44.6±21.7 & 35 & 0.713±0.002 & xx±xx & 0.719±0.002** \\
    \quad Schizophrenia & 24.0±2.9 & 50 & 0.838±0.003 & xx±xx & 0.860±0.006** \\
    \textbf{Pain treatment}  & 47.2±24.9 & 43 & 0.8078±0.0003 & xx±xx & 0.8222±0.0002*** \\
    \textbf{Pregnancy} \\
    \quad Preterm birth & 29.9±5.0 & 0 & 0.5337±0.0381 & xx±xx & 0.595±0.054 \\
    \quad FGR & 30.6±5.3 & 0 & 0.569±0.033 & xx±xx & 0.617±0.005* \\
    \quad Placental ins. & 32.0±6.0 & 0 & 0.588±0.010 & xx±xx & 0.586±0.022 \\
    \quad Large fetus & 31.4±4.9 & 0 & 0.579±0.054 & xx±xx & 0.616±0.055 \\
    \textbf{Others} \\
    \quad Sleep disorder & 29.9±5.8 & 48 & 0.748±0.002 & xx±xx & 0.759±0.002** \\
    \bottomrule
\end{tabular}
\end{table}

==> tables/main_table_v2.tex <==
\begin{table}[ht!]
\centering
 \caption{Model performance for base, base+ and best model for multiple conditions alongside age and prevalence for positive patients in the test set.\newline $^{*/**/***}\,$ Model is significantly better than base model $p<0.05/0.01/0.001$}
\begin{tabular}{p{0.23\linewidth}p{0.07\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.11\linewidth}p{0.11\linewidth}}
\toprule
Disease\newline(Age group/sex) & Age\newline Mean & Prevalence [\%] & AUROC base & AUROC base+ & AUROC best \\
\midrule
\textbf{Cancer} \\
\quad BCC ($70+$) & 80.1 & 4.57 & 0.644 & xx & 0.672** \\
\quad Breast ($60+$/f.) & 73.9 & 4.54 & 0.570 & xx & 0.624 \\
\quad Colon ($60+$) & 75.1 & 1.30 & 0.614 & xx & 0.628 \\
\quad Lung ($60+$) & 73.5 & 2.05 & 0.665 & xx & 0.684** \\
\quad Pancreas ($60+$) & 74.1 & 0.41 & 0.529 & xx & 0.565 \\
\textbf{Cardiovascular}\\
\quad Arrhythmia ($60+$) & 76.1 & 10.73 & 0.689 & xx & 0.716*** \\
\quad MI ($60+$) & 74.6 & 2.67 & 0.657 & xx & 0.687*** \\
\quad Stroke ($60+$) & 75.4 & 1.41 & 0.645 & xx & 0.702*** \\
\textbf{Chronic} \\
\quad AD ($70+$) & 81.6 & 3.68 & 0.739 & xx & 0.770*** \\
\quad Diabetes & 65.1 & 4.98 & 0.835 & xx & 0.848*** \\
\quad Osteonecrosis\newline($70+$) & 77.2 & 0.18 & 0.825 & xx & 0.842 \\
\textbf{Death} ($60+$) & 80.3 & 22.45 & 0.866 & xx & 0.877*** \\
\textbf{Emergencies} \\
\quad Anaphylaxis  & 32.1 & 0.16 & 0.710 & xx & 0.719 \\
\quad Diarrhea  & 59.0 & 1.32 & 0.856 & xx & 0.875** \\
\quad Major bleeding  & 59.3 & 4.69 & 0.782 & xx & 0.797*** \\
\textbf{Infections}  \\
\quad General & 46.8 & 42.61 & xx & xx & xx \\
\quad Pneumonia & 60.9 & 5.49 & 0.823 & xx & 0.832 \\
\textbf{Psychiatric} \\
\quad Depression\newline($15-30$) & 44.6 & 2.75 & 0.713 & xx & 0.719** \\
\quad Schizophrenia\newline($20-30$) & 24.0 & 1.15 & 0.838 & xx & 0.860** \\
\textbf{Pain treatment} & 47.2 & 42.04 & 0.808 & xx & 0.822*** \\
\textbf{Pregnancy} \\
\quad Preterm birth & 29.9 & 13.67 & 0.534 & xx & 0.595 \\
\quad FGR & 30.6 & 6.60 & 0.569 & xx & 0.617* \\
\quad Placental ins. & 32.0 & 0.58 & 0.588 & xx & 0.586 \\
\quad Large fetus& 31.4 & 2.26 & 0.579 & xx & 0.616 \\
\textbf{Others} \\
\quad Sleep disorder\newline($20-40$) & 29.9 & 4.30 & 0.748 & xx & 0.759** \\
\bottomrule
\end{tabular}
\end{table}
\clearpage

==> tables/main_table_v3.tex <==
\begin{table}[ht!]
\centering
 \caption{Model performance for base, base+ and best model for multiple conditions alongside age and patient numbers and prevalence for positive patients in the test set.\newline $^{*/**/***}\,$ Model is significantly better than base model $p<0.05/0.01/0.001$}
\begin{tabular}{p{0.34\linewidth}p{0.07\linewidth}p{0.17\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}}
\toprule
Disease\newline(Age group/sex) & Age\newline Mean & Patients\newline [thousands]/\newline Prevalence [\%] & AUROC base & AUROC base+ & AUROC best \\
\midrule
\textbf{Cancer} \\
\quad Basal Cell Carcinoma ($70+$) & 80 & 20.6/4.7 & 0.644 & xx & 0.672** \\
\quad Breast ($60+$/f.) & 74 & 13.5/4.4 & 0.570 & xx & 0.624 \\
\quad Colon ($60+$) & 75 & 35.5/1.3 & 0.614 & xx & 0.628 \\
\quad Lung ($60+$) & 74 & 35.0/2.3 & 0.665 & xx & 0.684** \\
\quad Pancreas ($60+$) & 74 & 37.7/0.5 & 0.529 & xx & 0.565 \\
\textbf{Cardiovascular}\\
\quad Arrhythmia ($60+$) & 76 & 35.5/10.7 & 0.689 & xx & 0.716*** \\
\quad Myocardial Infarction ($60+$) & 75 & 40.4/2.6 & 0.657 & xx & 0.687*** \\
\quad Stroke ($60+$) & 75 & 30.2/1.3 & 0.645 & xx & 0.702*** \\
\textbf{Chronic} \\
\quad Alzheimer’s Disease ($70+$) & 82 & 23.1/3.7 & 0.739 & xx & 0.770*** \\
\quad Diabetes & 65 & 107.4/4.9 & 0.835 & xx & 0.848*** \\
\quad Osteonecrosis ($70+$) & 77 & 25.7/0.2 & 0.825 & xx & 0.842 \\
\textbf{Death} ($60+$) & 80 & 35.0/22.7 & 0.866 & xx & 0.877*** \\
\textbf{Emergencies} \\
\quad Anaphylaxis & 32 & 169.1/0.2 & 0.710 & xx & 0.719 \\
\quad Diarrhea & 59 & 158.1/1.4 & 0.856 & xx & 0.875** \\
\quad Major bleeding & 59 & 162.6/4.6 & 0.782 & xx & 0.797*** \\
\textbf{Infections} \\
\quad General & 47 & 141.0/42.8 & xx & xx & xx \\
\quad Pneumonia & 61 & 146.6/5.5 & 0.823 & xx & 0.832 \\
\textbf{Psychiatric} \\
\quad Depression ($15-30$) & 45 & 142.7/1.8 & 0.713 & xx & 0.719** \\
\quad Schizophrenia ($20-30$) & 24 & 12.7/1.2 & 0.838 & xx & 0.860** \\
\textbf{Pain treatment} & 47 & 133.8/42.0 & 0.808 & xx & 0.822*** \\
\textbf{Pregnancy} \\
\quad Preterm birth & 30 & 11.1/13.7 & 0.534 & xx & 0.595 \\
\quad Fetal Growth Restriction & 31 & 11.1/6.9 & 0.569 & xx & 0.617* \\
\quad Placental ins. & 32 & 11.1/0.5 & 0.588 & xx & 0.586 \\
\quad Large fetus & 31 & 11.1/2.4 & 0.579 & xx & 0.616 \\
\textbf{Others} \\
\quad Sleep disorder ($20-40$) & 30 & 34.0/4.1 & 0.748 & xx & 0.759** \\
\bottomrule
\end{tabular}
\end{table}
\clearpage

==> tables/main_table_vMikkel2.tex <==
\begin{table}[ht!]
\centering
 \caption{Model performance for base, base+ and best model for multiple conditions alongside age and patient numbers and prevalence for positive patients in the test set.}
\begin{tabular}{
p{0.26\linewidth}
>{\centering\arraybackslash}p{0.145\linewidth}
>{\centering\arraybackslash}p{0.044\linewidth}
>{\centering\arraybackslash}p{0.144\linewidth}
p{0.25\linewidth}}
\toprule
Disease\newline(Age group/sex) & Forecast Horizon & Age\newline Mean & Patients\newline [thousands]\newline Prevalence[\%] & AUROC [\%] \tablefootnote[1]{$^{*/**/***}\,$ Model is significantly better than base model $p<0.05/0.01/0.001$\newline
\dgr Model is significantly better than BEHRT+ model $p<0.05$}\newline BEHRT/BEHRT+/\newline COREBEHRT \\
\midrule
\textbf{Cancer} \\
Basal Cell\newline Carcinoma ($70+$) & 1 year & 80 & 20.6/4.7 & 64.4/65.8**/\textbf{67.2}** \\
Breast ($60+$/f.) & 3 mo. & 74 & 13.5/4.4 & 57.0/57.6/\textbf{62.4} \\
Colon ($60+$) & 3 mo. & 75 & 35.5/1.3 & 61.4/\textbf{63.6}**/62.8 \\
Lung ($60+$) & 3 mo. & 74 & 35.0/2.3 & 66.5/67.9*/\textbf{68.4}** \\
Pancreas ($60+$) & 3 mo. & 74 & 37.7/0.5 & 52.9/\textbf{57.5}/56.5 \\
\textbf{Cardiovascular}\\
Arrhythmia ($60+$) & 6 mo. & 76 & 35.5/10.7 & 68.9/71.5***/\textbf{71.6}*** \\
MI ($60+$) & 14 days & 75 & 40.4/2.6 & 65.7/68.3***/\textbf{68.7}*** \\
Stroke ($60+$) & 14 d. & 75 & 30.2/1.3 & 64.5/xx/70.2*** \\
\textbf{Chronic} \\
AD ($70+$) & 3 mo. & 82 & 23.1/3.7 & 73.9/76.5**/\textbf{77.0}*** \\
Diabetes & 6 mo. & 65 & 107.4/4.9 & 83.5/\textbf{84.8}***/84.8*** \\
Osteonecrosis ($70+$) & 6 mo. & 77 & 25.7/0.2 & 82.5/\textbf{84.6}/84.2 \\
\textbf{Death} ($60+$) & 1 yr. & 80 & 35.0/22.7 & 86.6/87.5***/\textbf{87.7}***\dgr \\
\textbf{Emergencies} \\
Anaphylaxis & 24 hr. & 32 & 169.1/0.2 & 71.0/71.4/\textbf{71.9} \\
Diarrhea & 3 d. & 59 & 158.1/1.4 & 85.6/86.5**/\textbf{87.5}** \\
Major Bleeding & 24 hr. & 59 & 162.6/4.6 & 78.2/78.9**/\textbf{79.7}***\dgr \\
\textbf{Infections} \\
General Infections & 7 d. & 47 & 141.0/42.8 & xx/xx/xx \\
Pneumonia & 14 d. & 61 & 146.6/5.5 & 82.3/83.0***/\textbf{83.2}*** \\
\textbf{Psychiatric} \\
Depression ($15-30$) & 3 mo. & 45 & 142.7/1.8 & 71.3/71.8**/\textbf{71.9}** \\
Schizophrenia ($20-30$) & 3 mo. & 24 & 12.7/1.2 & 83.8/85.8**/\textbf{86.0}** \\
\textbf{Pain treatment} & 1 mo. & 47 & 133.8/42.0 & 80.8/xx/82.2*** \\
\textbf{Pregnancy-Related} \\
Preterm birth & at pregnancy & 30 & 11.1/13.7 & 53.4/54.5/\textbf{59.5} \\
FGR & at pregnancy & 31 & 11.1/6.9 & 56.9/xx/61.7* \\
Placental insufficiency & at pregnancy & 32 & 11.1/0.5 & 58.8/56.3/\textbf{58.6} \\
Large fetus & at pregnancy & 31 & 11.1/2.4 & 57.9/60.8/\textbf{61.6} \\
\textbf{Others} \\
Sleep disorder ($20-40$) & 3 mo. & 30 & 34.0/4.1 & 74.8/xx/75.9** \\
\bottomrule
\end{tabular}
\end{table}
\clearpage

==> tables/main_table_vMikkel3.tex <==
\begin{table}[ht!]
\centering
 \caption{Model performance for baseline (BEHRT), intermediate (\behrtdata) and final (\behrtbest) model for multiple conditions alongside average age at censoring, patient numbers, and prevalence for positive patients in the test set. If applicable, the selected age group and sex are given in parentheses.}
\begin{tabular}{
p{0.31\linewidth}|
>{\centering\arraybackslash}p{0.144\linewidth}|
>{\centering\arraybackslash}p{0.06\linewidth}|
p{0.02\linewidth}|
p{0.02\linewidth}|
p{0.01\linewidth}|
p{0.01\linewidth}|
p{0.01\linewidth}|
}
\toprule
Condition\newline(Age Group/Sex) & 
Prediction Window & 
Mean Age & 
A & B &
C & D & E \\
%\multicolumn{2}{>{\centering\arraybackslash}p{0.2\linewidth}}{Patients\newline [thousands]/\newline Prevalence[\%]} & 
%\multicolumn{3}{>{\centering\arraybackslash}p{0.2\linewidth}}{AUROC [\%]\newline BEHRT/\behrtdata /\newline\behrtbest} \\
\midrule
\textbf{Cancer} \\
Basal Cell Carcinoma ($70+$) & 1 yr. & 80 & 20.6 & 4.7 & 64.4 & 65.8** & \textbf{67.2}** \\
Breast ($60+$/f.) & 3 mo. & 74 & 13.5 & 4.4 & 57.0 & 57.6 & \textbf{62.4} \\
Colon ($60+$) & 3 mo. & 75 & 35.5 & 1.3 & 61.4 & \textbf{63.6}** & 62.8 \\
Lung ($60+$) & 3 mo. & 74 & 35.0 & 2.3 & 66.5 & 67.9* & \textbf{68.4}** \\
Pancreatic ($60+$) & 3 mo. & 74 & 37.7 & 0.5 & 52.9 & \textbf{57.5} & 56.5 \\
\textbf{Cardiovascular}\\
Arrhythmia ($60+$) & 6 mo. & 76 & 35.5 & 10.7 & 68.9 & 71.5*** & \textbf{71.6}*** \\
Myocardial Infarction ($60+$) & 14 d. & 75 & 40.4 & 2.6 & 65.7 & 68.3*** & \textbf{68.7}*** \\
Stroke ($60+$) & 14 d. & 75 & 30.2 & 1.3 & 64.5 & 69.4** & \textbf{70.2}*** \\
\textbf{Chronic} \\
Alzheimer’s Disease ($70+$) & 3 mo. & 82 & 23.1 & 3.7 & 73.9 & 76.5** & \textbf{77.0}*** \\
Diabetes & 6 mo. & 65 & 107.4 & 4.9 & 83.5 & \textbf{84.8}*** & \textbf{84.8}*** \\
Osteonecrosis ($70+$) & 6 mo. & 77 & 25.7 & 0.2 & 82.5 & \textbf{84.6} & 84.2 \\
\textbf{Death} ($60+$) & 1 yr. & 80 & 35.0 & 22.7 & 86.6 & 87.5*** & \textbf{87.7}***\dgr \\
\textbf{Emergencies} \\
Anaphylaxis & 24 hr. & 32 & 169.1 & 0.2 & 71.0 & 71.4 & \textbf{71.9} \\
Diarrhea & 3 d. & 59 & 158.1 & 1.4 & 85.6 & 86.5** & \textbf{87.5}**\dgr \\
Major Bleeding & 24 hr. & 59 & 162.6 & 4.6 & 78.2 & 78.9** & \textbf{79.7}***\dgr \\
\textbf{Infections} \\
General Infections & 7 d. & 47 & 141.0 & 42.8 & 78.2 & 79.7*** & \textbf{79.9}***\dgr \\
Pneumonia & 14 d. & 61 & 146.6 & 5.5 & 82.3 & 83.0*** & \textbf{83.2}***\dgr \\
\textbf{Psychiatric} \\
Depression ($15-30$) & 3 mo. & 45 & 142.7 & 1.8 & 71.3 & 71.8** & \textbf{71.9}** \\
Schizophrenia ($20-30$) & 3 mo. & 24 & 12.7 & 1.2 & 83.8 & 85.8** & \textbf{86.0}** \\
\textbf{Pain treatment} & 1 mo. & 47 & 133.8 & 42.0 & 80.8 & 82.1*** & \textbf{82.2}***\dgr\dgr \\
\textbf{Pregnancy-Related} \\
Preterm birth & at pregnancy & 30 & 11.1 & 13.7 & 53.4 & 54.5 & \textbf{59.5} \\
Fetal Growth Restriction & at pregnancy & 31 & 11.1 & 6.9 & 56.9 & 61.6*** & \textbf{61.7}*\dgr\dgr\dgr \\
Placental insufficiency & at pregnancy & 32 & 11.1 & 0.5 & \textbf{58.8} & 56.3 & 58.6 \\
Large fetus & at pregnancy & 31 & 11.1 & 2.4 & 57.9 & 60.8 & \textbf{61.6} \\
\textbf{Others} \\
Sleep disorder ($20-40$) & 3 mo. & 30 & 34.0 & 4.1 & 74.8 & \textbf{75.9**} & \textbf{75.9}** \\

\bottomrule
\multicolumn{5}{l}{\small{$^{*/**/***}\,$ Model is significantly better than BEHRT with $p<0.05/0.01/0.001$}}\\
\multicolumn{5}{l}{\small{\dgr\textsuperscript{/}\dgr\dgr\textsuperscript{/}\dgr\dgr\dgr\, Model is significantly better than \behrtdata with $p<0.05/0.01/0.001$}}
\end{tabular}\label{tab:results}
\end{table}
\clearpage


==> tables/max_performance.tex <==

\begin{table}
\caption{Results obtained with \behrtbest\:model for an increased cross-validation set on select conditions. AUROC is given with standard deviation computed from the five folds. The same test sets as described in \autoref{tab:results} was used.}
\label{tab:condition_stats_old}
\begin{tabular}{>{\raggedright\arraybackslash}p{0.34\linewidth} >{\centering\arraybackslash}p{0.18\linewidth} >{\centering\arraybackslash}p{0.18\linewidth} >{\centering\arraybackslash}p{0.18\linewidth}}
\toprule
Condition\newline(Age Group/Sex) & Patients in CV [thousands] & Prevalence [\%] & AUROC [\%] \\
\midrule
Breast Cancer ($60+$/f.) & 124.3 & 5.2 & 63.9$\pm$0.3 \\
Preterm Birth & 100.0 & 13.7 & 63.7$\pm$0.2 \\
Schizophrenia ($20-30$) & 89.2 & 1.4 & 85.9$\pm$0.6 \\
Stroke ($60+$) & 276.2 & 1.5 & 70.7$\pm$0.5 \\
\bottomrule
\end{tabular}
\end{table}




